Partition-based Feasible Integer Solution Pre-computation for Hybrid Model Predictive Control

For multiparametric mixed-integer convex programming problems such as those encountered in hybrid model predictive control, we propose an algorithm for generating a feasible partition of a subset of the parameter space. The result is a static map from the current parameter to a suboptimal integer solution such that the remaining convex program is feasible. Convergence is proven with a new insight that the overlap among the feasible parameter sets of each integer solution governs the partition complexity. The partition is stored as a tree which makes querying the feasible solution efficient. The algorithm can be used to warm start a mixed integer solver with a real-time guarantee or to provide a reference integer solution in several suboptimal MPC schemes. The algorithm is tested on randomly generated systems with up to six states, demonstrating the effectiveness of the approach.

==> phase2.tex <==
\section{Phase II: Computing $f_\delta^\epsilon$}
\label{sec:phase2}

This section presents the next and final phase of the algorithm in which
$f_\delta$ output by phase I is refined into the suboptimal commutation function
$f_\delta^\epsilon$. This is achieved by subdividing the phase I partition of
$\Theta$ further into simplices until an $\epsilon$-suboptimal $\delta$ choice
is found.

We begin by explaining the core logic step in the algorithm. Let
$(\mathcal R,\delta)$ be one of the cells of the phase I partition. We wish to
know whether $\delta$ is $\epsilon$-suboptimal in $\mathcal R$. This can be
encoded in the following two bilevel MINLPs for the absolute and relative errors
respectively:
\begin{align}
  \label{eq:absolute_error}
  e_{\mathrm{a}}^*(\mathcal R)
  &= \max_{\theta\in\mathcal R,\delta'\in\binary^m\setminus\{\delta\}}
    V_\delta^*(\theta)-V_{\delta'}^*(\theta),
    \tag{E$^{\mathcal R}_{\mathrm{a}}$} \\
  \label{eq:relative_error}
  e_{\mathrm{r}}^*(\mathcal R)
  &= \max_{\theta\in\mathcal R,\delta'\in\binary^m\setminus\{\delta\}}
    (V_\delta^*(\theta)-V_{\delta'}^*(\theta))/V_{\delta'}^*(\theta).
    \tag{E$^{\mathcal R}_{\mathrm{r}}$}
\end{align}
If $e_{\mathrm{a}}^*(\mathcal R)\le\epsilon_{\mathrm{a}}$ or
$e_{\mathrm{r}}^*(\mathcal R)\le\epsilon_{\mathrm{r}}$ then, according to
Definition~\ref{definition:suboptimal_commutation_function}, $\delta$ is
$\epsilon$-suboptimal in $\mathcal R$. Both problems, however, are non-convex
and as such their globally optimal solution is not readily
obtainable. Nevertheless, we can formulate a tractable alternative optimization
that is \textit{sufficient} to guarantee
$e_{\mathrm{a}}^*(\mathcal R)\le\epsilon_{\mathrm{a}}$ or
$e_{\mathrm{r}}^*(\mathcal R)\le\epsilon_{\mathrm{r}}$. We focus first on
$e_{\mathrm{a}}^*(\mathcal R)$.

\begin{definition}
  Let $v_i\in\mathcal V(\mathcal R)$ be the $i$-th vertex of $\mathcal R$ and
  let $\theta=\sum_{i=1}^{|\mathcal V(\mathcal R)|}\alpha_iv_i$,
  $\sum_{i=1}^{|\mathcal V(\mathcal R)|}\alpha_i=1$ and $\alpha_i\ge 0$
  $\forall i=1:|\mathcal V(\mathcal R)|$. The affine over-approximator
  over $\mathcal R$ of $V^*_\delta(\theta)$ is:
  \begin{equation}
    \label{eq:over_approximator}
    \bar V_\delta(\theta)\triangleq\sum_{i=1}^{|\mathcal V(\mathcal R)|}\alpha_iV^*_\delta(v_i).
  \end{equation}
\end{definition}

\begin{proposition}
  \label{proposition:over_approximator}
  The affine over-approximator (\ref{eq:over_approximator}) satisfies
  $V^*_{\delta}(\theta)\le\bar V_{\delta}(\theta)$ $\forall\theta\in\mathcal R$
  and with equality at the vertices.
  \begin{proof}
    Since $V^*_{\delta}$ is convex (Lemma~\ref{lemma:convexity}), Jensen's
    inequality implies $V^*_\delta(\theta)\le\bar V_\delta(\theta)$.
  \end{proof}
\end{proposition}

Consider now the following convex MINLP:
\begin{equation}
  \label{eq:absolute_error_approx}
  \bar e_{\mathrm{a}}(\mathcal R)
  =
  \max_{\theta\in\mathcal R,\delta'\in\binary^m\setminus\{\delta\}}
  \bar V_\delta(\theta)-V^*_{\delta'}(\theta)
  \tag{$\bar{\text{E}}^{\mathcal R}_{\mathrm{a}}$}
\end{equation}

\begin{lemma}
  \label{lemma:absolute_error}
  The error measures satisfy
  $e^*_{\mathrm{a}}(\mathcal R)\le \bar e_{\mathrm{a}}(\mathcal R)$.
  \begin{proof}
    Let $\theta\in\mathcal R$ and $\delta'\in\binary^m\setminus\{\delta\}$. By
    Proposition~\ref{proposition:over_approximator},
    $V^*_\delta(\theta)\le\bar V_\delta(\theta)\Rightarrow V^*_\delta(\theta)-V^*_{\delta'}(\theta)\le\bar V_\delta(\theta)-V^*_{\delta'}(\theta)$. The
    result follows directly.
  \end{proof}
\end{lemma}

\begin{theorem}
  \label{theorem:absolute_error_check_sufficiency}
  Verifying $\bar e_{\mathrm{a}}(\mathcal R)\le\epsilon_{\mathrm{a}}$ is a
  sufficient for
  $e_{\mathrm{a}}^*(\mathcal R)\le\epsilon_{\mathrm{a}}$ to hold.
  \begin{proof}
    By Lemma~\ref{lemma:absolute_error},
    $e_{\mathrm{a}}^*(\mathcal R)\le\bar e_{\mathrm{a}}(\mathcal R)\le\epsilon_{\text{a}}$.
  \end{proof}
\end{theorem}

As a tractable alternative to (\ref{eq:relative_error}), we suggest the
following tractable over-approximation \cite{MunozDeLaPena2004}:
\begin{equation*}
  \label{eq:relative_error_approx}
  \bar e_{\mathrm{r}}(\mathcal R) = \frac{
    \bar e_{\mathrm{a}}(\mathcal R)
  }{
    \min_{\theta\in\mathcal R}V^*_\delta(\theta)
  }.
  \tag{$\bar{\text{E}}^{\mathcal R}_{\mathrm{r}}$}
\end{equation*}

Evidently, $e_{\mathrm{r}}^*(\mathcal R)\le \bar e_{\mathrm{r}}(\mathcal R)$.
As for the absolute error, we have the following theorem.

\begin{theorem}
  \label{theorem:relative_error_check_sufficiency}
  Verifying $\bar e_{\mathrm{r}}(\mathcal R)\le\epsilon_{\mathrm{r}}$ is a
  sufficient for
  $e_{\mathrm{r}}^*(\mathcal R)\le\epsilon_{\mathrm{r}}$ to hold.
  \begin{proof}
    We have
    $e_{\mathrm{r}}^*(\mathcal R)\le\bar e_{\mathrm{r}}(\mathcal R)\le\epsilon_{\text{r}}$.
  \end{proof}
\end{theorem}

The result of Theorems~\ref{theorem:absolute_error_check_sufficiency} and
\ref{theorem:relative_error_check_sufficiency} is that the intractable
(\ref{eq:absolute_error}) and (\ref{eq:relative_error}) can be substituted for
the tractable (\ref{eq:absolute_error_approx}) and
(\ref{eq:relative_error_approx}) in order to guarantee the
$\epsilon$-suboptimality requirement. Note that because $\epsilon$-suboptimality
checks only for $\delta'\in\binary^m\setminus\{\delta\}$, it is less stringent
than requiring it for all $\delta\in\binary^m$. While in the former case
partitioning stops as soon as the sufficient conditions are met, the latter case
would partition all the way until $V^*_\delta$ is sufficient accurately
approximated. The result is a coarser partition and is thanks to our
semi-explicit programming approach.

When both $\bar e_{\mathrm{a}}(\mathcal R)>\epsilon_{\mathrm{a}}$ and
$\bar e_{\mathrm{r}}(\mathcal R)>\epsilon_{\mathrm{r}}$, however, nothing can be
said as to whether $e_{\mathrm{a}}^*(\mathcal R)\le\epsilon_{\text{a}}$. In this
case, the algorithm will subdivide $\mathcal R$ in order to decrease the
over-approximation error
$\max_{\theta\in\mathcal R}\bar V_\delta(\theta)-V^*_\delta(\theta)$.

We now propose Algorithm~\ref{alg:phase2} to compute $f_\delta^\epsilon$. Aside
from $\epsilon_{\mathrm{a}}$ and $\epsilon_{\mathrm{r}}$, the algorithm requests
$\bar\rho$, the maximum tolerated simplex condition number. Given
$v_i\in\mathcal V(\mathcal R)$ where $\mathcal R\subset\reals^p$ is a simplex,
the condition number is given by:
\begin{equation}
  \label{eq:condition_number}
  \rho(\mathcal R)\triangleq\frac{\overline\sigma(
    \begin{bmatrix}
      v_2-v_1 & \cdots & v_{p+1}-v_1
    \end{bmatrix}
    )}{
    \underline\sigma(
    \begin{bmatrix}
      v_2-v_1 & \cdots & v_{p+1}-v_1
    \end{bmatrix}
    )},
\end{equation}
where $\overline\sigma$ and $\underline\sigma$ are the largest and smallest
singular values respectively. Since Algorithm~\ref{alg:phase1} cannot produce
lower-dimensional simplices, no division by zero can occur in
(\ref{eq:condition_number}). Through $\bar\rho$, Algorithm~\ref{alg:phase2}
takes the practical approach of giving up the $\epsilon$-suboptimality guarantee
in very badly conditions cells. If $\bar\rho$ is large, $\epsilon$-suboptimality
will eventually be guaranteed everywhere but numerics may become sensitive and
the partition complexity prohibitive. By reducing the $\bar\rho$ value, the
partition will be computed more quickly by neglecting a few cells where further
partitioning will cause $\rho(\mathcal R)>\bar\rho$. In our experience, a good
$\bar\rho$ setting yields $<1\%$ of such cells in the final partition (see
Section~\ref{sec:example}).

The algorithm also requires parameters $\pi_{\mathrm{a}}$ and $\pi_{\mathrm{r}}$
which define the absolute and relative keep-out radii by which
$\bar\theta_{\mathrm{a}}(\mathcal R)$, the arg-maximizer of
(\ref{eq:absolute_error_approx}), has to be away from any
$v\in\mathcal V(\mathcal R)$. Practical experience has shown that if
$\exists v\in\mathcal V(\mathcal R)$ such that
$\|v-\bar\theta_{\mathrm{a}}(\mathcal R)\|_2$ is very small, the partitioning
process slows down significantly. In this case Algorithm~\ref{alg:phase2}
prefers to partition $\mathcal R$ along the midpoint of its longest edge, which
is a heuristic that we have found to work well when $\mathcal R$ needs to be
split but $\theta^*_{\mathrm{a}}(\mathcal R)$ cannot be split at due to
$\pi_{\mathrm{a}}$ or $\pi_{\mathrm{r}}$.

\begin{algorithm}[t]
  \centering
  \begin{algorithmic}[1]
    \State Open all leaves of tree output by Algorithm~\ref{alg:phase1}
    \While{any open leaf exists}
    \For{every open leaf $(\mathcal R,\delta)$}
    \If{$\mathcal R$ is not a simplex}
    \label{alg:phase2:line:polytosimplex}
    \State $\mathcal S\gets\mathtt{delaunay}(\mathcal V(\mathcal R))$
    \State Add child open leaves $(\mathcal S_i,\delta)$
    $\forall\mathcal S_i\in\mathcal S$
    \label{alg:phase2:line:polytosimplexend}
    \Else
    \State $\bar e_{\mathrm{a}}(\mathcal R)\gets\text{solve
      (\ref{eq:absolute_error_approx})}$
    \label{alg:phase2:line:suboptimalitycheckstart}
    \State $\bar e_{\mathrm{r}}(\mathcal R)\gets\text{solve
      (\ref{eq:relative_error_approx})}$
    \State $\text{infeasible}\gets\text{(\ref{eq:absolute_error_approx}) or (\ref{eq:relative_error_approx})
      infeasible}$
    \State $\text{$\epsilon$-suboptimal}\gets\text{$\bar e_{\mathrm{a}}(\mathcal R)\le\epsilon_{\mathrm{a}}$ or
      $\bar e_{\mathrm{r}}(\mathcal R)\le\epsilon_{\mathrm{r}}$}$
    \If{infeasible or $\epsilon$-suboptimal}
    \State Close leaf
    \label{alg:phase2:line:suboptimalitycheckend}
    \Else
    \State $\bar l\gets\max_{v,v'\in\mathcal V(\mathcal R)}\|v-v'\|_2$
    \State $r_{\text{ko}}\gets\max\{\pi_{\mathrm{a}},\pi_{\mathrm{r}}\bar l\}$
    \State
    $\bar\theta_{\mathrm{a}}(\mathcal R),\bar\delta_{\mathrm{a}}(\mathcal R)\gets\arg\max\text{
    of (\ref{eq:absolute_error_approx})}$
    \If{$\|\bar\theta_{\mathrm{a}}(\mathcal R)-v\|_2>r_{\text{ko}}$
      $\forall v\in\mathcal V(\mathcal R)$}
    \State
    $\bar v,\bar v'\gets\arg\max_{v,v'\in\mathcal V(\mathcal R)}\|v-v'\|_2$
    \label{alg:phase2:line:edgesplit}
    \State
    $\mathcal S\gets\mathtt{triangulate}(\mathcal R,(\bar v+\bar v')/2)$
    \If{$\exists \mathcal S_i\in\mathcal S$ such that $\rho(\mathcal S_i)>\bar\rho$}
    \State Close leaf with warning
    \label{alg:phase2:line:suboptimalclose}
    \EndIf
    \Else
    \State
    $\mathcal S\gets\mathtt{triangulate\_snap}(\bar V_\delta,\mathcal R,\bar\delta_{\mathrm{a}}(\mathcal R))$
    \If{$|\mathcal S|=1$}
    \State \Goto{alg:phase2:line:edgesplit}
    \EndIf
    \EndIf
    \For{each $\mathcal S_i\in\mathcal S$}
    \label{alg:phase2:line:changecommutation}
    \If{(\ref{eq:nlp}) feas. for $\delta=\bar\delta_{\mathrm{a}}(\mathcal R)$,
      $\forall\theta\in\mathcal V(\mathcal S_i)$}
    \State Add child open leaf $(\mathcal S_i,\bar\delta_{\mathrm{a}}(\mathcal R))$
    \Else
    \State Add child open leaf $(\mathcal S_i,\delta)$
    \EndIf
    \EndFor
    \EndIf
    \EndIf
    \EndFor
    \EndWhile
    \label{alg:phase2:line:end}
    \caption{Phase II computation of $f_\delta^{\epsilon}$.}
    \label{alg:phase2}
  \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
  \centering
  \begin{algorithmic}[1]
    \Function{$\mathtt{triangulate\_snap}$}{$V$,$\mathcal R$,$\delta$}
    \State Denote $\mathcal V(\mathcal R)=\{v_1,\dots,v_{\ell}\}$
    \State $c\gets v_{\ell},E\gets 
    \setlength\arraycolsep{1pt}
    \begin{bmatrix}
      v_1-v_{\ell} & \cdots & v_p-v_{\ell}
    \end{bmatrix}$
    \label{alg:snap:line:basis}
    \State $\theta'\gets\text{solve
      (\ref{eq:absolute_error_approx_constrained})}$
    \State
    $\mathcal S\gets\mathtt{triangulate}(\mathcal R,\theta')$
    \State $i\gets\arg\max_{i=1,\dots,|\mathcal S|}\rho(\mathcal S_i)$
    \If{$\rho(\mathcal S_i)>\bar\rho$}
    \State $\text{facet}_i\gets \Co(\mathcal V(\mathcal S_i)\setminus\{\theta'\})$
    \State $\mathcal S\gets\mathtt{triangulate\_snap}(V,\text{facet}_i,\delta)$
    \State $v\gets\mathcal V(\mathcal R)\setminus\text{facet}_i$
    \State $\mathcal S\gets\{\Co(\mathcal V(\mathcal D)\cup\{v\}):\mathcal D\in\mathcal S\}$
    \EndIf
    \State \Return $\mathcal S$
    \EndFunction
    \caption{Condition number-aware triangulation.}
    \label{alg:triangulate_snap}
  \end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:phase2} proceeds as follows. First, all leaves of the tree
output by Algorithm~\ref{alg:phase1} are re-opened for further
partitioning. Lines~\ref{alg:phase2:line:polytosimplex}-\ref{alg:phase2:line:end}
partition the cell $(\mathcal R,\delta)$. Because Algorithm~\ref{alg:phase1} can
return general polytopes, these are first partitioned via Delaunay triangulation
on
lines~\ref{alg:phase2:line:polytosimplex}-\ref{alg:phase2:line:polytosimplexend}. When
$\mathcal R$ is a simplex, the sufficient conditions provided by
Theorems~\ref{theorem:absolute_error_check_sufficiency} and
\ref{theorem:relative_error_check_sufficiency} are used to check
$\epsilon$-suboptimality on
lines~\ref{alg:phase2:line:suboptimalitycheckstart}-\ref{alg:phase2:line:suboptimalitycheckend}. If
$\delta$ is the only feasible commutation in $\mathcal R$,
(\ref{eq:absolute_error_approx}) and (\ref{eq:relative_error_approx}) will
fail. In this case, $\delta$ is certainly the optimal commutation as it is the
only feasible one. However, if $\epsilon$-suboptimality is not verified,
$\mathcal R$ must be further partitioned. We first check that the point of
maximum suboptimality $\bar\theta_{\mathrm{a}}(\mathcal R)$ is away from any
vertex by the aforementioned keep-out radius. If not, $\mathcal R$ is
partitioned into two simplices at the midpoint of its longest edge where
$\mathtt{triangulate}(\mathcal S,\theta)$ partitions $\mathcal S$ into
$\{\mathcal S'=\Co((\mathcal V(\mathcal S)\setminus v)\cup\{\theta\}):v\in\mathcal V(\mathcal S),\mathcal S'\text{
  full-dimensional}\}$. If the resulting simplices exceed the condition number
tolerance, $\mathcal R$ is not partitioned and is closed on
line~\ref{alg:phase2:line:suboptimalclose} with a warning that
$\bar e_{\mathrm{a}}(\mathcal R)>\epsilon_{\mathrm{a}}$ and
$\bar e_{\mathrm{r}}(\mathcal R)>\epsilon_{\mathrm{r}}$.

Line~\ref{alg:phase2:line:suboptimalclose} is the only case where the
user-requested $\epsilon$-suboptimality is not achieved and deserves
justification. First, we note that by setting $\bar\rho$ large enough, one can
cause line~\ref{alg:phase2:line:suboptimalclose} to never be visited. However,
two practical issues may prevent arbitrarily large $\bar\rho$ settings: 1) badly
conditioned simplices can cause failure due to numerical precision error and 2)
bad conditioning is symptomatic of a prohibitively complex partitioning
resulting from too small $\epsilon_{\mathrm{a}}$ or $\epsilon_{\mathrm{r}}$. In
this respect, $\bar\rho$ is advantageous because in practice the partition
complexity required by a certain $\epsilon_{\mathrm{a}}$ and
$\epsilon_{\mathrm{r}}$ cannot be known a priori
\cite{MunozDeLaPena2004}. Thanks to $\bar\rho$, however, excessive partitioning
is abandoned and one can check post factum the \textit{achieved}
$\bar e_{\mathrm{a}}(\mathcal R)$ and $\bar e_{\mathrm{r}}(\mathcal R)$ for all
leaves of the partition tree. One can then either increase $\bar\rho$ or accept
the achieved values.

When $\bar\theta_{\mathrm{a}}(\mathcal R)$ passes the keep-out check,
$\mathcal R$ is partitioned at $\bar\theta_{\mathrm{a}}(\mathcal R)$ via
Algorithm~\ref{alg:triangulate_snap}. On line~\ref{alg:snap:line:basis}, a basis
of convex set $\mathcal R$, which is at most a simplex, is constructed. The
point at which to split $\mathcal R$ is then obtained by solving a
fixed-commutation maximum absolute error NLP on the affine set $\Range(E)+c$:
\begin{equation}
  \label{eq:absolute_error_approx_constrained}
  \optimize[
  \theta=E\alpha+c \\
  &&& \alpha\ge 0,\text{ }\textstyle{\sum}_{i=1}^\ell\alpha_i=1.
  ]{\theta_{\delta}(c,E,V)}{\arg\max}{\alpha,\theta}{V(\theta)-V_\delta^*(\theta)}
  \tag{$\bar{\text{E}}_{\mathrm{a}}^{\delta,c,E,V}$}
\end{equation}

It may happen, however, that $\theta_{\delta}(c,E,V)$ is close to some, for
example, a facet of $\mathcal R$ at which point $\mathtt{triangulate}$ will
return at least one very badly conditioned simplex. In this situation, we
identify the worst-conditioned simplex in the triangulation of $\mathcal R$ and
re-run $\mathtt{triangulate\_snap}$ on the lower-dimensional polytope formed by
the vertices of $\mathcal R$ associated with the worst-conditioned simplex. This
recursion returns either some well-conditioned partition of $\mathcal R$ or, if
solving the lower-dimensional problems did not help to improve the condition
number, $\mathcal R$ itself. In the latter case, Algorithm~\ref{alg:phase2}
falls back to the longest edge midpoint partitioning heuristic. With the
partition $\mathcal S$ of $\mathcal R$ obtained,
lines~\ref{alg:phase2:line:changecommutation}-\ref{alg:phase2:line:end} of
Algorithm~\ref{alg:phase2} create new open leaves for each cell $\mathcal S$
with the associated commutation $\bar\delta_{\mathrm{a}}(\mathcal R)$ whenever
possible. In situations where it turns out that
$\bar\delta_{\mathrm{a}}(\mathcal R)$ is feasible at
$\bar\theta_{\mathrm{a}}(\mathcal R)$ but not
$\forall v\in\mathcal V(\mathcal R)$, the leaf is created with the original
$\delta$ and we rely on the partitioning process to eventually assign the
$\epsilon$-suboptimal commutation.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "root"
%%% End:

